Analysis of the South Slavic Scripts by Run-Length Features of the Image Texture

The paper proposes an algorithm for the script recognition based on the texture characteristics. The image texture is achieved by coding each letter with the equivalent script type (number code) according to its position in the text line. Each code is transformed into equivalent gray level pixel creating an 1-D image. Then, the image texture is subjected to the run-length analysis. This analysis extracts the run-length features, which are classified to make a distinction between the scripts under consideration. In the experiment, a custom oriented database is subject to the proposed algorithm. The database consists of some text documents written in Cyrillic, Latin and Glagolitic scripts. Furthermore, it is divided into training and test parts. The results of the experiment show that 3 out of 5 run-length features can be used for effective differentiation between the analyzed South Slavic scripts.

==> refs.tex <==
\begin{thebibliography}{10}

\bibitem{Amelio2014}
A.~Amelio and C.~Pizzuti.
\newblock A new evolutionary-based clustering framework for image databases.
\newblock In Abderrahim Elmoataz, Olivier Lezoray, Fathallah Nouboud, and Driss
  Mammass, editors, {\em Image and Signal Processing}, volume 8509 of {\em
  Lecture Notes in Computer Science}, pages 322--331. Springer International
  Publishing, 2014.

\bibitem{Brodic2013}
D.~Brodi\'c, Z.N. Milivojevi\'c, and C.A. Maluckov.
\newblock Recognition of the script in serbian documents using frequency
  occurrence and co-occurrence analysis.
\newblock {\em The Scientific World Journal}, 2013, no. 896328:1--14, 2013.

\bibitem{Brodic2014}
D.~Brodi\'c, Z.N. Milivojevi\'c, and C.A. Maluckov.
\newblock An approach to the script discrimination in the slavic documents.
\newblock {\em Soft Computing}, pages 1--11, 2014.

\bibitem{Busch2005}
A.~Busch, W.W. Boles, and S.~Sridharan.
\newblock Texture for script identification.
\newblock {\em Pattern Analysis and Machine Intelligence, IEEE Transactions
  on}, 27(11):1720--1732, Nov 2005.

\bibitem{Galloway75}
M.M. Galloway.
\newblock Texture analysis using gray level run lengths.
\newblock {\em Computer Graphics and Image Processing}, 4(2):172 -- 179, 1975.

\bibitem{Gho2010}
D.~Ghosh, T.~Dube, and A.P. Shivaprasad.
\newblock Script recognition - a review.
\newblock {\em Pattern Analysis and Machine Intelligence, IEEE Transactions
  on}, 32(12):2142--2161, Dec 2010.

\bibitem{Jain95}
R.~Jain, R.~Kasturi, and B.G. Schunck.
\newblock {\em Machine Vision}.
\newblock McGraw-Hill, Inc., New York, NY, USA, 1995.

\bibitem{Joshi2007}
G.D. Joshi, S.~Garg, and J.~Sivaswamy.
\newblock A generalised framework for script identification.
\newblock {\em {IJDAR}}, 10(2):55--68, 2007.

\bibitem{Kast2002}
R.~Kasturi, L.~O'Gorman, and V.~Govindaraju.
\newblock Document image analysis: A primer.
\newblock {\em Sadhana}, 27(1):3--22, 2002.

\bibitem{Pal2002}
U.~Pal and B.B Chaudhuri.
\newblock Identification of different script lines from multi-script documents.
\newblock {\em Image and Vision Computing}, 20(13–14):945 -- 954, 2002.

\bibitem{Sovi2014}
S.~Sovilj-Nikic, D.~Delic Vlado, I.B. Sovilj-Nikic, and M.~Markovic.
\newblock Tree-based phone duration modelling of the serbian language.
\newblock {\em ELEKTRONIKA IR ELEKTROTECHNIKA}, 20(3):77--82, 2014.

\bibitem{Srin2008}
G.~N. Srinivasan and G.~Shobha.
\newblock Statistical texture analysis.
\newblock In {\em Proceedings of World Academy of Science, Engineering and
  Technology}, volume~36, pages 1264--1269, 2008.

\bibitem{Tang98}
X.~Tang.
\newblock Texture information in run-length matrices.
\newblock {\em Image Processing, IEEE Transactions on}, 7(11):1602--1609, Nov
  1998.

\bibitem{Xu2004}
D.~Xu, A.S. Kurani, J.D. Furst, and D.S. Raicu.
\newblock Run-length encoding for volumetric texture.
\newblock In {\em The 4th IASTED International Conference on Visualization,
  Imaging, and Image Processing}, 2004.

\bibitem{Zram98}
A.~Zramdini and R.~Ingold.
\newblock Optical font recognition using typographical features.
\newblock {\em Pattern Analysis and Machine Intelligence, IEEE Transactions
  on}, 20(8):877--882, Aug 1998.

\end{thebibliography}

